Attention Prompting on Image for Large Vision-Language Models

Compared with Large Language Models (LLMs), Large Vision-Language Models (LVLMs) can also accept images as input, thus showcasing more interesting emergent capabilities and demonstrating impressive performance on various vision-language tasks. Motivated by text prompting in LLMs, visual prompting has been explored to enhance LVLMs' capabilities of perceiving visual information. However, previous visual prompting techniques solely process visual inputs without considering text queries, limiting the models' ability to follow text instructions to complete tasks. To fill this gap, in this work, we propose a new prompting technique named Attention Prompting on Image, which just simply overlays a text-query-guided attention heatmap on the original input image and effectively enhances LVLM on various tasks. Specifically, we generate an attention heatmap for the input image dependent on the text query with an auxiliary model like CLIP. Then the heatmap simply multiplies the pixel values of the original image to obtain the actual input image for the LVLM. Extensive experiments on various vison-language benchmarks verify the effectiveness of our technique. For example, Attention Prompting on Image improves LLaVA-1.5 by 3.8% and 2.9% on MM-Vet and LLaVA-Wild benchmarks, respectively.

==> 2Table/cls_non_cls.tex <==
\begin{table}[tb]
  \caption{Comparison between using the $\Psi^{cls}$ and $\Psi^{comp}$.
  }
  \label{tab:abl1}
  \centering
\begin{tabular}{@{}cccccccc@{}}
\toprule
               &  &                                  &                   & \multicolumn{2}{c}{Query: ``Where is the desk?''} & \multicolumn{2}{c}{Query: ``Where is the blanket?''} \\ \cmidrule(l){5-8} 
               &  &                                  &                   & Annotated Image               & Mask              & Annotated Image                & Mask                \\ \midrule
Original Image & \includegraphics[width=1cm]{3Figure/cls_non_cls/v1_122.jpg} & \multirow{2}{*}{Annotated Image} & Use $\Psi^{cls}$  &                               &                   &                                &                     \\
               &  &                                  & Use $\Psi^{comp}$ &                               &                   &                                &                     \\ \bottomrule
\end{tabular}
\end{table}
